Improving Calibration in Deep Metric Learning With Cross-Example Softmax

Modern image retrieval systems increasingly rely on the use of deep neural networks to learn embedding spaces in which distance encodes the relevance between a given query and image. In this setting, existing approaches tend to emphasize one of two properties. Triplet-based methods capture top-$k$ relevancy, where all top-$k$ scoring documents are assumed to be relevant to a given query Pairwise contrastive models capture threshold relevancy, where all documents scoring higher than some threshold are assumed to be relevant. In this paper, we propose Cross-Example Softmax which combines the properties of top-$k$ and threshold relevancy. In each iteration, the proposed loss encourages all queries to be closer to their matching images than all queries are to all non-matching images. This leads to a globally more calibrated similarity metric and makes distance more interpretable as an absolute measure of relevance. We further introduce Cross-Example Negative Mining, in which each pair is compared to the hardest negative comparisons across the entire batch. Empirically, we show in a series of experiments on Conceptual Captions and Flickr30k, that the proposed method effectively improves global calibration and also retrieval performance.

==> CES NeurIPS/abstract.tex <==
% While these randomness affects the learned weights, does it also affect the final predictions?

Standard training techniques for neural networks involve multiple sources of randomness, e.g., initialization, mini-batch ordering and in some cases data augmentation. Given that neural networks are heavily over-parameterized in practice, such randomness can cause {\em churn} -- disagreements between predictions of the two models independently trained by the same algorithm, contributing to the `reproducibility challenges' in modern machine learning. In this paper, we study this problem of churn, identify factors that cause it, and propose two simple means of mitigating it. We first demonstrate that churn is indeed an issue, even for standard image classification tasks (CIFAR and ImageNet), and study the role of the different sources of training randomness that cause churn. By analyzing the relationship between churn and prediction confidences, we pursue two strategies for churn reduction. First, we propose using \emph{minimum entropy regularizers} to increase prediction confidences. Second, we study \emph{co-distillation} \citep{zhang2018deep, anil2018large}, a technique proposed to increase model agreement. We present empirical results showing the effectiveness of both techniques in reducing churn while improving the accuracy of the underlying model.

%In this paper, we study the disagreement between predictions of different instances of neural network trained using the same randomized learning algorithm, referred to as \emph{churn}. 
%We measure churn for some standard image classification tasks and show that indeed models have a significant disagreement in their predictions across runs, and study the role of the different sources of randomness in training that cause churn. 

%In this paper we study the problem of prediction stability of neural networks. We analyze the disagreement between predictions of models, a.k.a churn,   


==> CES NeurIPS/appx_experiments.tex <==
\section{Additional experimental results}
%
\begin{figure}[!p]
    \centering
    \includegraphics[scale=0.75]{figs/entropic_log_loss.pdf}
    \includegraphics[scale=0.75]{figs/entropic_logistic_loss.pdf}
    \caption{Visualisation of entropic regularised loss in binary case.
    On the left panel is the regularised log-loss $-\log p + \alpha \cdot H_{\mathrm{bin}}( p )$, which accepts a probability in $[0, 1]$ as input.
    On the right panel is the logistic loss $-\log \sigma( f ) + \alpha \cdot H_{\mathrm{bin}}( \sigma( f ) )$, which accepts a score in $\mathbb{R}$ as input and passes it through sigmoid $\sigma( \cdot )$ to get a probability estimate.}
    \label{fig:loss_visualisation}
\end{figure}

%
\begin{figure}[!p]
    \centering
    \includegraphics[scale=0.75]{figs/kl_log_loss_v2.pdf}
    \includegraphics[scale=0.75]{figs/kl_logistic_loss_v2.pdf}
    \caption{Visualisation of KL-regularised loss in binary case.
    On the left panel is the regularised log-loss $(1-\alpha) \cdot -\log p + \alpha \cdot \mathrm{KL}( \mathrm{Unif} \| p )$, which accepts a probability in $[0, 1]$ as input.
    On the right panel is the logistic loss $(1-\alpha) \cdot -\log \sigma( f ) + \alpha \cdot \mathrm{KL}( \mathrm{Unif} \| \sigma( f ) )$, which accepts a score in $\mathbb{R}$ as input and passes it through sigmoid $\sigma( \cdot )$ to get a probability estimate.}
    \label{fig:loss_visualisation_v2}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.35]{figs/histlogits0_32.png}
    \includegraphics[scale=0.35]{figs/histlogits5_32.png}
    \caption{\cifarT{}, \resnetT{}. Histogram of logits for models trained with KL regularizer $\alpha=0$ and $\alpha=0.3$ .}
    \label{fig:entropy_logits}
\end{figure}


\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.35]{figs/hist0_32.png}
    \includegraphics[scale=0.35]{figs/hist5_32.png}
    \caption{\cifarT{}, \resnetT{}. Histogram of L1, L1normalized and L4 distance for models trained with KL regularizer $\alpha=0$ and $\alpha=0.3$ .}
    \label{fig:smooth_dist}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.45]{figs/smoothed_comparison.png}
    \includegraphics[scale=0.45]{figs/smoothed_half.png}
    \caption{\cifarT{}, \resnetT{}. Comparison of pairwise churn, $L_1$ and $L_{0.5}$ normalized dist.}
    \label{fig:comparison}
\end{figure}

\begin{figure}[hbpt]
    \centering
    \includegraphics[scale=0.45]{figs/anectodal_p.png}
    \includegraphics[scale=0.45]{figs/anectodal_n.png}
    \caption{\cifarT{}, \resnetT{}. Predictions of models trained with KL regularizer $\alpha=0$ vs $\alpha=0.3$. The regularizer improves prediction stability for both correct and incorrect predictions.}
    \label{fig:anecdotal}
\end{figure}


==> CES NeurIPS/header.tex <==
\usepackage{amsmath,amsfonts,amssymb,amsthm, color}
\usepackage{algorithm,algorithmicx}
\usepackage{epsfig,wrapfig,epsf,subcaption}
\usepackage[outercaption]{sidecap} 
\usepackage{times}
\usepackage{fancyvrb}
\usepackage{enumerate}
\usepackage{tikz}
\usepackage{bm}
\usetikzlibrary{arrows,shapes}
\usetikzlibrary{patterns}
\usepackage{graphicx}
\usepackage{comment}
%\usepackage{fullpage}
\usepackage{ltxtable}
\usepackage{nicefrac}
\usepackage{multirow}
\usepackage{setspace}
%\usepackage[colorlinks=true, linkcolor=black, bookmarks=true]{hyperref}
\usepackage[noend]{algpseudocode}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{microtype}      % microtypographysubsection
\usepackage{pbox}
\usepackage{xfrac}

\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\corref}[1]{Corollary~\ref{#1}}
\newcommand{\assumpref}[1]{Assumption~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}


%\renewcommand{\eqref}[1]{Eq.~(\ref{#1})}
%\newcommand{\subsecref}[1]{Subsection~\ref{#1}}
%\newcommand{\exref}[1]{Example~\ref{#1}}

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{condition}{Condition}
\newtheorem{remark}[theorem]{Remark}
\newreptheorem{theorem}{Theorem}
\newreptheorem{lemma}{Lemma}
\newreptheorem{definition}{Definition}
\newenvironment{sketch}{\paragraph{Proof sketch}\mbox{}}{\hfill $\blacksquare$}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{question}{Question}
\newtheorem*{answer}{Answer}


\newcommand{\intenum}{\setcounter{saveenumi}{\theenumi}}
\newcommand{\contenum}{\setcounter{enumi}{\thesaveenumi}}
\newcounter{saveenumi}

\newcommand{\etal}{{\it et al}}



==> CES NeurIPS/notation.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%
\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}


% Random variables (\mathsf{})
\def\U{{\mathsf{U}}}
\def\V{{\mathsf{V}}}
\def\W{{\mathsf{W}}}
\def\X{{\mathsf{X}}}
\def\Y{{\mathsf{Y}}}
\def\Z{{\mathsf{Z}}}


% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\TV}{D_{\mathrm{TV}}}
\newcommand{\hellinger}[1]{D_\mathrm{hellinger}(#1)}
\newcommand{\hellingerS}[1]{D_\mathrm{hellinger}^2(#1)}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\churnA}[1]{\mathrm{Churn}_{#1}(\mathfrak{A})}
\newcommand{\churnAp}[1]{\mathrm{Churn}^{{\rm pair}, m}_{#1}(\mathfrak{A})}
\newcommand{\churnAova}[1]{\mathrm{Churn}^{{\rm ova}, m}_{#1}(\mathfrak{A})}
\newcommand{\churn}[1]{\mathrm{Churn}(#1)}
\newcommand{\schurn}[1]{\mathrm{SChurn}_{\alpha}(#1)}
\newcommand{\schurnnoarg}{\mathrm{SChurn}_{\alpha}}
\newcommand{\churnR}[1]{\mathrm{Churn}^{\rm rand}(#1)}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\perr}[1]{\mathrm{P}_{\rm Err, #1}}
\newcommand{\schurno}[1]{\mathrm{SChurn}_{1}(#1)}
\newcommand{\schurnt}[1]{\mathrm{SChurn}_{2}(#1)}

\newcommand{\cifar}{CIFAR}
\newcommand{\cifarT}{CIFAR-10}
\newcommand{\cifarH}{CIFAR-100}
\newcommand{\imagenet}{ImageNet}
\newcommand{\resnetT}{ResNet-32}
\newcommand{\resnetF}{ResNet-56}
\newcommand{\resnetIM}{ResNet-v2-50}


\newcommand{\model}[1]{f (#1 ; w)}
\newcommand{\modelO}[1]{f (#1 ; w_1)}
\newcommand{\modelT}[1]{f (#1 ; w_2)}
\newcommand{\modelp}[2]{f (#1 ; #2)}
\newcommand{\modelE}[1]{f (#1 ; \widetilde{w})}
\newcommand{\modelB}[1]{f (#1 ; w^*)}
\newcommand{\entropy}{\mathit{H}}
\newcommand{\abs}[1]{\left \vert #1 \right \vert}
\def\expec{{\mathbb{E}}}


\newcommand{\algo}[1]{\mathfrak{A}(#1)}

\newcommand{\todo}[1]{
  \textcolor{blue}{\textbf{TODO:} {#1}}
}

==> CES NeurIPS/reject.tex <==
\section{Classification with a reject option}

Consider the setting of binary classification with a reject option~\citep{Bartlett:2008}.
Specifically, for a given rejection cost $d > 0$ and rejection threshold $\delta$,
we are interested in minimising~\citep[Equation 1]{Bartlett:2008}
$$ R_{d, \delta}( f ) = \Pr( y \cdot f( x ) < -\delta ) + d \cdot \Pr( | y \cdot f( x ) | \leq \delta ). $$
This corresponds to using a rejection loss
$$ \ell_{d, \delta}( z ) = \begin{cases}
1 & \text{ if } z < -\delta \\
d & \text{ if } | z | \leq \delta \\
0 & \text{ else. }
\end{cases} $$
The Bayes-optimal classifier under this loss has the form~\citep[Equation 2]{Bartlett:2008}
\begin{equation}
\label{eqn:bayes-reject}
    f^*_{d}( x ) = \begin{cases}
    +1 & \text{ if } \eta( x ) > 1 - d \\
    0 & \text{ if } d \leq \eta( x ) \leq 1 - d \\
    -1 & \text{ else, }
\end{cases}
\end{equation}
where $\eta( x ) = \Pr( y = 1 \mid x )$.

A tight convex upper bound to this loss was provided in~\citet[Section 2]{Bartlett:2008}:
$$ \phi_{d}( z ) = \begin{cases}
1 - a \cdot z & \text{ if } z < 0 \\
1 - z & \text{ if } 0 \leq z < 1 \\
0 & \text{ else. }
\end{cases} $$
We may construct a smooth approximation to this loss via\footnote{This is derived in a straightforward manner: we first compute $\phi'_d( z )$; approximate the resulting indicator functions with sigmoids; and then integrate the result.}
$$ \bar{\phi}_{d, \alpha}( z ) = \frac{1}{\alpha} \cdot \left( (a - 1) \cdot \log( 1 + e^{\alpha \cdot z} ) + \log (1 + e^{\alpha - \alpha \cdot z}) \right) - (a - 1) \cdot z $$
where $\alpha \geq 1$.
An elementary calculation reveals that $\bar{\phi}_{d, \alpha} \to \phi_d$ pointwise as $\alpha \to \infty$.
This is visualised in Figure~\ref{fig:reject_logistic_loss}.

Note that the loss corresponds to using the log-loss in conjunction with the link
$$ \bar{F}_{d, \alpha}( z ) = \frac{(1 - a) \cdot \sigma(\alpha \cdot v) - \sigma(\alpha \cdot v + \alpha)}{(1 - a) - \sigma(\alpha \cdot v + \alpha) - \sigma(-\alpha \cdot v + \alpha)}. $$
% Observe that when $\alpha = 1$ and $d = \frac{1}{2}$ (so $a = 1$),
% $$ \bar{F}_{d, \alpha}( z ) = \frac{\sigma(z) - \sigma(- z - 1)}{1 - \sigma( z - 1 ) - \sigma(- z - 1)}. $$
We visualise this link for $d = 0.3$ and varying choices of $\alpha$ in Figure~\ref{fig:reject_logistic_link}.
As expected, when $\alpha$ grows larger, the link has a saturating behaviour around $\bar{F}_{d, \alpha}( z ) \in [ 0.3, 0.7 ]$.
As a consequence, under this loss,
the Bayes-optimal predictions in this range will saturate around $0$ when $\eta( x )$ is in this interval, and $\pm 1$ when outside this interval;
i.e.,
they converge to the Bayes-optimal predictions for the rejection loss in Equation~\ref{eqn:bayes-reject}.
This is verified in Figure~\ref{fig:reject_logistic_inv_link}.

%
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.5]{figs/reject_logistic_loss.pdf}
    \caption{Loss function $\bar{\phi}_{d, \alpha}( z )$ for $d = 0.3$ and various values of $\alpha$.}
    \label{fig:reject_logistic_loss}
\end{figure}

%
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.5]{figs/reject_logistic_link.pdf}
    \caption{Link function $\bar{F}_{d, \alpha}( z )$ for $d = 0.3$ and various values of $\alpha$.}
    \label{fig:reject_logistic_link}
\end{figure}

%
\begin{figure}[!t]
    \centering
    
    \subfloat[Original axes.]{\includegraphics[scale=0.375]{figs/reject_logistic_inv_link.pdf}}%
    \quad%
    \subfloat[Zoomed in axes .]{\includegraphics[scale=0.375]{figs/reject_logistic_inv_link_zoomed.pdf}}
    
    \caption{Bayes-optimal predictions under the proposed loss for $d = 0.3$ and various values of $\alpha$.
    Observe that for $\eta( x ) \in [0.3, 0.7]$, the optimal prediction converges to 0.
    For $\eta( x ) > 0.7$, the optimal solution converges to $+1$,
    while for $\eta( x ) < 0.3$, the optimal solution converges to $-1$.
    This is in agreement with the desired optimal solution in Figure~\ref{eqn:bayes-reject}.}
    \label{fig:reject_logistic_inv_link}
\end{figure}

==> CES NeurIPS/todo.tex <==
%
\section{Todo}
Evolution during training, Ablation, 10 runs for all exp?, imagenet examples, another vision dataset?, LM?, 
\begin{itemize}
\item Define and demonstrate Churn. 
    \begin{itemize}
        \item Define (soft) churn.
        \item Demonstrate churn on different datasets and architectures.
        \begin{itemize}
            \item CIFAR10, Imagenet, WMT14. 
            \item FF, Convnet, Resnet, Transformers.
            \item Linear models?
        \end{itemize}
        \item Figure out the small L1 distance on Imagenet.
    \end{itemize}
    
    \item What factors cause it?
    \begin{itemize}
        \item \textbf{random initialization}
        \item \textbf{mini batch ordering}
        \item always the same subset of examples?
        \item input preprocessing (random crop/scale/etc)?
        \item momentum vs adam?
        \item batch normalization?
    \end{itemize}
    
    \item Connection to other stability/reproducibility notions
    
    \item Solutions
    \begin{itemize}
        \item \textbf{entropy and kl regularizers }
        \begin{itemize}
            \item constant regularizers
            \item schedule
        \end{itemize}
        \item \textbf{scaling softmax temperature }
        \item reject option
        \begin{itemize}
            \item Reject CE/hinge loss and its connections to margin penalty
            \item Boosting, reject loss vs distillation. They seem to have opposite effects on hard examples.
        \end{itemize}
        \item ensembling; why does it help?
        \item \textbf{dropout as implicit ensembling}
        \item mixup
        \item loss + label smoothing
        \begin{itemize}
            \item Square loss
            \item Softmax + square loss
            \item Generalised cross-entropy
            \item Margin loss
        \end{itemize}
        \item lottery ticket and solution paths
        \item smooth activations?
        \item how to penalize initialization part orthogonal to data manifold?
    \end{itemize}
\end{itemize}

\section{Outline}
\begin{itemize}
\item Churn: Is it a significant problem? What is it caused by?
    \item Boundary examples. Are they really confusing or a artifact of the model/training procedure?
    \item Classification with reject option.
    \item new regularizer?
\end{itemize}
\clearpage


==> abstract.tex <==
% While these randomness affects the learned weights, does it also affect the final predictions?

Standard training techniques for neural networks involve multiple sources of randomness, e.g., initialization, mini-batch ordering and in some cases data augmentation. Given that neural networks are heavily over-parameterized in practice, such randomness can cause {\em churn} -- disagreements between predictions of the two models independently trained by the same algorithm, contributing to the `reproducibility challenges' in modern machine learning. In this paper, we study this problem of churn, identify factors that cause it, and propose two simple means of mitigating it. We first demonstrate that churn is indeed an issue, even for standard image classification tasks (CIFAR and ImageNet), and study the role of the different sources of training randomness that cause churn. By analyzing the relationship between churn and prediction confidences, we pursue two strategies for churn reduction. First, we propose using \emph{minimum entropy regularizers} to increase prediction confidences. Second, we study \emph{co-distillation} \citep{zhang2018deep, anil2018large}, a technique proposed to increase model agreement. We present empirical results showing the effectiveness of both techniques in reducing churn while improving the accuracy of the underlying model.

%In this paper, we study the disagreement between predictions of different instances of neural network trained using the same randomized learning algorithm, referred to as \emph{churn}. 
%We measure churn for some standard image classification tasks and show that indeed models have a significant disagreement in their predictions across runs, and study the role of the different sources of randomness in training that cause churn. 

%In this paper we study the problem of prediction stability of neural networks. We analyze the disagreement between predictions of models, a.k.a churn,   


==> appx_experiments.tex <==
\section{Additional experimental results}
%
\begin{figure}[!p]
    \centering
    \includegraphics[scale=0.75]{figs/entropic_log_loss.pdf}
    \includegraphics[scale=0.75]{figs/entropic_logistic_loss.pdf}
    \caption{Visualisation of entropic regularised loss in binary case.
    On the left panel is the regularised log-loss $-\log p + \alpha \cdot H_{\mathrm{bin}}( p )$, which accepts a probability in $[0, 1]$ as input.
    On the right panel is the logistic loss $-\log \sigma( f ) + \alpha \cdot H_{\mathrm{bin}}( \sigma( f ) )$, which accepts a score in $\mathbb{R}$ as input and passes it through sigmoid $\sigma( \cdot )$ to get a probability estimate.}
    \label{fig:loss_visualisation}
\end{figure}

%
\begin{figure}[!p]
    \centering
    \includegraphics[scale=0.75]{figs/kl_log_loss_v2.pdf}
    \includegraphics[scale=0.75]{figs/kl_logistic_loss_v2.pdf}
    \caption{Visualisation of KL-regularised loss in binary case.
    On the left panel is the regularised log-loss $(1-\alpha) \cdot -\log p + \alpha \cdot \mathrm{KL}( \mathrm{Unif} \| p )$, which accepts a probability in $[0, 1]$ as input.
    On the right panel is the logistic loss $(1-\alpha) \cdot -\log \sigma( f ) + \alpha \cdot \mathrm{KL}( \mathrm{Unif} \| \sigma( f ) )$, which accepts a score in $\mathbb{R}$ as input and passes it through sigmoid $\sigma( \cdot )$ to get a probability estimate.}
    \label{fig:loss_visualisation_v2}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.35]{figs/histlogits0_32.png}
    \includegraphics[scale=0.35]{figs/histlogits5_32.png}
    \caption{\cifarT{}, \resnetT{}. Histogram of logits for models trained with KL regularizer $\alpha=0$ and $\alpha=0.3$ .}
    \label{fig:entropy_logits}
\end{figure}


\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.35]{figs/hist0_32.png}
    \includegraphics[scale=0.35]{figs/hist5_32.png}
    \caption{\cifarT{}, \resnetT{}. Histogram of L1, L1normalized and L4 distance for models trained with KL regularizer $\alpha=0$ and $\alpha=0.3$ .}
    \label{fig:smooth_dist}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.45]{figs/smoothed_comparison.png}
    \includegraphics[scale=0.45]{figs/smoothed_half.png}
    \caption{\cifarT{}, \resnetT{}. Comparison of pairwise churn, $L_1$ and $L_{0.5}$ normalized dist.}
    \label{fig:comparison}
\end{figure}

\begin{figure}[hbpt]
    \centering
    \includegraphics[scale=0.45]{figs/anectodal_p.png}
    \includegraphics[scale=0.45]{figs/anectodal_n.png}
    \caption{\cifarT{}, \resnetT{}. Predictions of models trained with KL regularizer $\alpha=0$ vs $\alpha=0.3$. The regularizer improves prediction stability for both correct and incorrect predictions.}
    \label{fig:anecdotal}
\end{figure}


==> reject.tex <==
\section{Classification with a reject option}

Consider the setting of binary classification with a reject option~\citep{Bartlett:2008}.
Specifically, for a given rejection cost $d > 0$ and rejection threshold $\delta$,
we are interested in minimising~\citep[Equation 1]{Bartlett:2008}
$$ R_{d, \delta}( f ) = \Pr( y \cdot f( x ) < -\delta ) + d \cdot \Pr( | y \cdot f( x ) | \leq \delta ). $$
This corresponds to using a rejection loss
$$ \ell_{d, \delta}( z ) = \begin{cases}
1 & \text{ if } z < -\delta \\
d & \text{ if } | z | \leq \delta \\
0 & \text{ else. }
\end{cases} $$
The Bayes-optimal classifier under this loss has the form~\citep[Equation 2]{Bartlett:2008}
\begin{equation}
\label{eqn:bayes-reject}
    f^*_{d}( x ) = \begin{cases}
    +1 & \text{ if } \eta( x ) > 1 - d \\
    0 & \text{ if } d \leq \eta( x ) \leq 1 - d \\
    -1 & \text{ else, }
\end{cases}
\end{equation}
where $\eta( x ) = \Pr( y = 1 \mid x )$.

A tight convex upper bound to this loss was provided in~\citet[Section 2]{Bartlett:2008}:
$$ \phi_{d}( z ) = \begin{cases}
1 - a \cdot z & \text{ if } z < 0 \\
1 - z & \text{ if } 0 \leq z < 1 \\
0 & \text{ else. }
\end{cases} $$
We may construct a smooth approximation to this loss via\footnote{This is derived in a straightforward manner: we first compute $\phi'_d( z )$; approximate the resulting indicator functions with sigmoids; and then integrate the result.}
$$ \bar{\phi}_{d, \alpha}( z ) = \frac{1}{\alpha} \cdot \left( (a - 1) \cdot \log( 1 + e^{\alpha \cdot z} ) + \log (1 + e^{\alpha - \alpha \cdot z}) \right) - (a - 1) \cdot z $$
where $\alpha \geq 1$.
An elementary calculation reveals that $\bar{\phi}_{d, \alpha} \to \phi_d$ pointwise as $\alpha \to \infty$.
This is visualised in Figure~\ref{fig:reject_logistic_loss}.

Note that the loss corresponds to using the log-loss in conjunction with the link
$$ \bar{F}_{d, \alpha}( z ) = \frac{(1 - a) \cdot \sigma(\alpha \cdot v) - \sigma(\alpha \cdot v + \alpha)}{(1 - a) - \sigma(\alpha \cdot v + \alpha) - \sigma(-\alpha \cdot v + \alpha)}. $$
% Observe that when $\alpha = 1$ and $d = \frac{1}{2}$ (so $a = 1$),
% $$ \bar{F}_{d, \alpha}( z ) = \frac{\sigma(z) - \sigma(- z - 1)}{1 - \sigma( z - 1 ) - \sigma(- z - 1)}. $$
We visualise this link for $d = 0.3$ and varying choices of $\alpha$ in Figure~\ref{fig:reject_logistic_link}.
As expected, when $\alpha$ grows larger, the link has a saturating behaviour around $\bar{F}_{d, \alpha}( z ) \in [ 0.3, 0.7 ]$.
As a consequence, under this loss,
the Bayes-optimal predictions in this range will saturate around $0$ when $\eta( x )$ is in this interval, and $\pm 1$ when outside this interval;
i.e.,
they converge to the Bayes-optimal predictions for the rejection loss in Equation~\ref{eqn:bayes-reject}.
This is verified in Figure~\ref{fig:reject_logistic_inv_link}.

%
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.5]{figs/reject_logistic_loss.pdf}
    \caption{Loss function $\bar{\phi}_{d, \alpha}( z )$ for $d = 0.3$ and various values of $\alpha$.}
    \label{fig:reject_logistic_loss}
\end{figure}

%
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.5]{figs/reject_logistic_link.pdf}
    \caption{Link function $\bar{F}_{d, \alpha}( z )$ for $d = 0.3$ and various values of $\alpha$.}
    \label{fig:reject_logistic_link}
\end{figure}

%
\begin{figure}[!t]
    \centering
    
    \subfloat[Original axes.]{\includegraphics[scale=0.375]{figs/reject_logistic_inv_link.pdf}}%
    \quad%
    \subfloat[Zoomed in axes .]{\includegraphics[scale=0.375]{figs/reject_logistic_inv_link_zoomed.pdf}}
    
    \caption{Bayes-optimal predictions under the proposed loss for $d = 0.3$ and various values of $\alpha$.
    Observe that for $\eta( x ) \in [0.3, 0.7]$, the optimal prediction converges to 0.
    For $\eta( x ) > 0.7$, the optimal solution converges to $+1$,
    while for $\eta( x ) < 0.3$, the optimal solution converges to $-1$.
    This is in agreement with the desired optimal solution in Figure~\ref{eqn:bayes-reject}.}
    \label{fig:reject_logistic_inv_link}
\end{figure}

==> todo.tex <==
%
\section{Todo}
Evolution during training, Ablation, 10 runs for all exp?, imagenet examples, another vision dataset?, LM?, 
\begin{itemize}
\item Define and demonstrate Churn. 
    \begin{itemize}
        \item Define (soft) churn.
        \item Demonstrate churn on different datasets and architectures.
        \begin{itemize}
            \item CIFAR10, Imagenet, WMT14. 
            \item FF, Convnet, Resnet, Transformers.
            \item Linear models?
        \end{itemize}
        \item Figure out the small L1 distance on Imagenet.
    \end{itemize}
    
    \item What factors cause it?
    \begin{itemize}
        \item \textbf{random initialization}
        \item \textbf{mini batch ordering}
        \item always the same subset of examples?
        \item input preprocessing (random crop/scale/etc)?
        \item momentum vs adam?
        \item batch normalization?
    \end{itemize}
    
    \item Connection to other stability/reproducibility notions
    
    \item Solutions
    \begin{itemize}
        \item \textbf{entropy and kl regularizers }
        \begin{itemize}
            \item constant regularizers
            \item schedule
        \end{itemize}
        \item \textbf{scaling softmax temperature }
        \item reject option
        \begin{itemize}
            \item Reject CE/hinge loss and its connections to margin penalty
            \item Boosting, reject loss vs distillation. They seem to have opposite effects on hard examples.
        \end{itemize}
        \item ensembling; why does it help?
        \item \textbf{dropout as implicit ensembling}
        \item mixup
        \item loss + label smoothing
        \begin{itemize}
            \item Square loss
            \item Softmax + square loss
            \item Generalised cross-entropy
            \item Margin loss
        \end{itemize}
        \item lottery ticket and solution paths
        \item smooth activations?
        \item how to penalize initialization part orthogonal to data manifold?
    \end{itemize}
\end{itemize}

\section{Outline}
\begin{itemize}
\item Churn: Is it a significant problem? What is it caused by?
    \item Boundary examples. Are they really confusing or a artifact of the model/training procedure?
    \item Classification with reject option.
    \item new regularizer?
\end{itemize}
\clearpage

